Can LLMs Speak For Diverse People? Tuning LLMs via Debate to Generate Controllable Controversial Statements

Making LLMs speak for different, especially minority groups of people, and generate statements supporting their diverse or even controversial perspectives is critical to creating an inclusive environment. However, existing LLMs lack sufficient controllability to the stance of their generated content, which often contains inconsistent, neutral, or biased statements. In this paper, we improve the controllability of LLMs in generating statements supporting an argument the user defined in the prompt. We find that multi-round debates between two LLMs with opposite stances generate higher-quality and more salient statements for each, which are important training data to improve the controllability of LLMs. Motivated by this, we develop a novel debate & tuning (DEBATUNE) pipeline finetuning LLMs to generate the statements obtained via debate. To examine DEBATUNE, we curate the largest dataset of debate topics so far, which covers 710 controversial topics and corresponding arguments for each topic. Evaluations by the GPT-4 judge with a novel controversy controllability metric show that LLMs' capability of generating diverse perspectives is significantly improved by DEBATUNE. Moreover, such controllability can be generalized to unseen topics, generating high-quality statements supporting controversial arguments.

==> Figures/figure_intro_1.tex <==
\begin{figure}[!t]
\centering 
\includegraphics[width=0.5\textwidth]{Figures/intro.png} 
\caption{
A controversial example that includes the user query and the responses generated by different models. For the controversial topic ``Organ donation should be mandatory'', the user would like to get a controllable response with a negative stance with respect to ``Religious and cultural objections''. (a) The existing model is not able to stick to the controlled stance and begins to express its own preference, i.e. positive. (b) Our model is able to stick to the controllable stance during a whole generation of responses. 
} 
\label{intro} 
\end{figure}


==> statistic_evaluation.tex <==


\subsection{Controllable Diversity}

As shown in Figure \ref{intro}, one problem of the current LLMs is the lack of controllability and diversity, possibly influenced by the pretraining corpus, they tend to output similar statements even in a totally different stance. The motivation of our method is to train a model with controllability, which can generate in-depth statements on either the stance or argument of a controversial debate topic. Thus we propose an evaluation method for the evaluation of this controllable diversity. 

Our evaluation method lies on a hypothesis: \textbf{Under the same topic, the similarity of statements belonging to different stances is supposed to be less than the statements of the same stance.} For example, the similarity of two statements that both support the topic should be relatively higher, as they share the same high-level viewpoint, even though the specific statements are different. On the contrary, the similarity of statements that have different stances should be smaller, as they support the opposite side of a topic. 

Specifically, we utilize the cosine similarity of the sentence embeddings as the measurement of the similarity between two statements, which can be notated as cos$(\cdot)$. Let $f$ denote the pretrained language model for calculating sentence embeddings, then for two statements $y_1$ and $y_2$, the conscience similarity value $v$ can be notated as:
\begin{equation}
     v = \text{sim}(y_1, y_2) = \text{cos}(g(y_1),g(y_2))
\end{equation} 

Suppose there are $k$ different arguments for each stance $p_{t}$ or $n_{t}$ of a topic $t$, then the averaged similarity $\Bar{v}_{p_t, p_t}$ of sentence pair within the positive stance $p_t$ can be notated as:  
\begin{equation}
     \Bar{v}_{p_t, p_t} = \frac{1}{k(k - 1)} \sum_{i=1}^{k} \sum_{j=1,i \neq j }^{k} \text{sim}(y_{p_{t}, i}, y_{p_{t}, j})
\end{equation} 
Similarly, the averaged similarity $\Bar{v}_{n_t, n_t}$ of sentence pair within the negative stance $n_t$ can be noted similarly. 

Except for the intra-stance similarity, the averaged similarity between arguments with different stances $\Bar{v}_{p_t, n_t}$ is also vital as it directly measures the discrepancy between contrastive arguments. For an LLM that is able to generate opposite in-depth statements, this similarity score should be small, as they stand for the direct exclusive sides, which can be notated as:
\begin{equation}
     \Bar{v}_{p_t, n_t} = \frac{1}{k_1 \cdot k_2} \sum_{i=1}^{k_1} \sum_{j=1}^{k_2} \text{sim}(y_{p_{t}, i}, y_{n_{t}, j})
\end{equation} 
where $k_1$ and $k_2$ represent the number of statements for $p_t$ and $n_t$, respectively. 

Though these cosine similarity values to some extent can directly reflect the diversity of responses, their absolute values vary largely for different LLMs, due to their diverse data distributions and training strategies, making it hard to be a general evaluation metric. Thus to solve this problem, we propose to calculate the ratio $r_t$ between similarities of the same and different stances for topic $t$:
\begin{equation}
     r_t = \frac{\Bar{v}_{p_t, p_t} + \Bar{v}_{n_t, n_t}}{2\cdot \Bar{v}_{p_t, n_t}}
\end{equation} 
We name this ratio as Controversy Diversity score (CD score) for simplicity as it directly measures how much diversity the model can produce when generating statements for controversial topics. The averaged CD scores $\Bar{r_t}$ across the whole test set can be a general static measurement that suits most LLMs. When the CD score is less than $1$, it represents that the statement similarities of different stances are even larger than the similarities within the same stances, which is undesirable and unreasonable. On the contrary, when the CD score is larger than $1$ or higher, it indicates a greater gap between the intra- and inter-similarities, indicating that LLM can generate more divergent responses when changing the stances, further indicating better controllability. 


\begin{table}[!tbh]
\centering
\scalebox{0.84}{
\begin{tabular}{lcccc}
\hline
& $\Bar{v}_{p, p}$ & $\Bar{v}_{n, n}$ & $\Bar{v}_{p, n}$ & CD score \\\hline
Alpaca 7B & 0.985 & 0.983 & 0.982 & 1.002     \\ 
WizardLM 7B & 0.972 & 0.987 & 0.969 & 1.011     \\ 
Vicuna 7B v1.5 & 0.958 & 0.970 & 0.950 & 1.015     \\ 
Vicuna 13B v1.5 & 0.987 & 0.988 & 0.977 & 1.011     \\ 
LLaMA2 Chat 7B & 0.985 & 0.986 & 0.981 & 1.005     \\ 
LLaMA2 Chat 13B & 0.979 & 0.982 & 0.979 & 1.002     \\ 
sRecycled Wiz 7B & 0.967 & 0.967 & 0.963 & 1.004     \\ 
Zephyr 7B Alpha & 0.992 & 0.991 & 0.989 & 1.003     \\ 
Zephyr 7B Beta & 0.972 & 0.973 & 0.958 & 1.015     \\ 
% ChatGPT & -     & -       & - & -     \\
\hline
Ours & 0.994 & 0.996 & 0.959 & 1.038 \\ 
\hline
\end{tabular}
}
\caption{
The Controllable Diversity scores on controversial debate topics of existing LLMs. 
}
\label{tbl:ablation}
\end{table}

